A Hierarchical Recurrent Encoder-Decoder For Generative Context-Aware Query Suggestion

Users may strive to formulate an adequate textual query for their information need. Search engines assist the users by presenting query suggestions. To preserve the original search intent, suggestions should be context-aware and account for the previous queries issued by the user. Achieving context awareness is challenging due to data sparsity. We present a probabilistic suggestion model that is able to account for sequences of previous queries of arbitrary lengths. Our novel hierarchical recurrent encoder-decoder architecture allows the model to be sensitive to the order of queries in the context while avoiding data sparsity. Additionally, our model can suggest for rare, or long-tail, queries. The produced suggestions are synthetic and are sampled one word at a time, using computationally cheap decoding techniques. This is in contrast to current synthetic suggestion models relying upon machine learning pipelines and hand-engineered feature sets. Results show that it outperforms existing context-aware approaches in a next query prediction setting. In addition to query suggestion, our model is general enough to be used in a variety of other applications.

==> 01-intro.tex <==
% !TEX root =  cikm2015-sordonia.tex

%Web user queries are usually short, ambiguous or under-specified.
%Users may be searching for information in domains they are not familiar with. 
%Or, they may be engaged in an exploratory search task covering multiple aspects of the same topic. 
%In this cases, it is difficult to find an adequate textual representation to satisfy the information need. 
%As a result, the search experience may be unsatisfactory and time-consuming.
%To overcome this issue, modern search engines heavily assist the users in their search task by providing query suggestions.
%Query auto-completion suggestions help users to complete their queries while they are typing in the search box, i.e. based on the current %prefix.
%In this paper, we focus on the task of generating query reformulation suggestions, i.e. alternative query reformulations that are computed once that one or more queries have already been submitted to the search engine. 
%Web user queries are usually short, ambiguous or under-specified. 
%As a result, users may find their search experience unsatisfactory and time-consuming. 
%A query suggestion system provide alternative textual queries once that one or more queries have already been submitted by a user.
%Web search engines heavily rely on query suggestions to support users during their search tasks.

Web user queries are usually short, ambiguous or under-specified. 
Users may be searching for information in domains they are not familiar with. 
Or, they may be engaged in an exploratory search task covering multiple aspects of the same topic. 
In this cases, it is difficult to formulate an adequate textual representation to satisfy the information need. 
As a result, the search experience may be unsatisfactory and time-consuming.
Modern search engines heavily rely on query suggestions to support users during their search task. Auto-completion suggestions help users to complete their queries while they are typing in the search box. In this paper, we focus on query reformulation suggestions, that are produced after one or more queries have already been submitted to the search engine. 

Search query logs are an important resource to mine user reformulation behaviour. The query log is partitioned into query sessions, i.e.~sequences of queries issued by a unique user and submitted within a short time interval.  A query session contains the sequence of query reformulations issued by the user while attempting to complete the search mission. Therefore, query co-occurrence in the same session is a strong signal of query relatedness and can be straightforwardly used to produce suggestions.

Methods solely relying on query co-occurrence are prone to data sparsity and lack coverage for rare and \emph{long-tail} queries, i.e.~unseen in the training data.
A suggestion system should be able to translate infrequent queries to more common and effective formulations based on similar queries that have been seen in the training data. 
To do so, some models capture capture higher order collocations~\cite{Boldi2008}, consider additional resources~\cite{Jain2011,Vahabi2013}, move towards a word-level representation~\cite{Bonchi2012,Broccolo2012} or describe queries using a rich feature space and apply learning to rank techniques to select meaningful candidates~\cite{Ozertem2012,Santos2013}. 

An additional desirable property of a suggestion system is \emph{context-awareness}. 
Pairwise suggestion system operate by considering only the most recent query.
However, previous submitted queries provide useful context to narrow down ambiguity in the current query and to produce more focused suggestions~\cite{Jiang2014}. 
Equally important is the order in which past queries are submitted, as it denotes generalization or specification reformulation patterns~\cite{Huang2009}. A major hurdle for current context-aware models is dealing with the dramatic growth of diverse contexts, since it induces sparsity, and classical count-based models become unreliable~\cite{Cao2008,He2009}.

%Consider the following example: a user initiates the search task by submitting the query \emph{san felipe}, then submits \emph{costa azul} and finally concludes with \emph{costa azul hotel san felipe}. The concept of \emph{san felipe} is plainly motivated by the first query. Accounting for the second query only may generate suggestions that are topically too broad for the current user.

Finally, relatively unexplored for suggestion systems is the ability to produce \emph{synthetic} suggestions. 
Typically, we assume that useful suggestions are already present in the training data. 
The assumption weakens for rare queries or complex information needs, for which it is possible that the best suggestion has not been previously seen~\cite{Jain2011, Templates11}. 
In these cases, synthetic suggestions can be leveraged to increase coverage and can be used as candidates in complex learning to rank models~\cite{Ozertem2012}.

We present a probabilistic model capable of generating synthetic, context-aware suggestions in the long-tail.
It acts as a language model of query sessions, represented as sequences of words interleaved with a special end-of-query token.
Given a sequence of queries as prefix, it predicts the most likely sequence of words that follow the prefix. 
Variable contexts can be accounted for without strict built-in length limits.
Query suggestions can be mined by sampling likely continuations given one or more queries as context.
Prediction is cheap and can be performed using standard natural language processing word-level decoding techniques~\cite{Koehn2009}.
A suggestion is produced when the special end-of-query token appears in the samples.
As an example, given a context of two queries \emph{cleveland gallery}~$\circ$~\emph{lake erie art}~$\circ$, where $\circ$ denotes the end-of-query symbol, our model continues the session by sampling sequentially the words \emph{cleveland}, \emph{indian}, \emph{art} and $\circ$. As the end-of-query token has been reached, the completion given by our model is \emph{cleveland gallery}~$\circ$~\emph{lake erie art} $\circ$ \emph{cleveland indian art} $\circ$.
The last query represents a generated synthetic suggestion. The model is robust to long-tail effects as the prefix is considered as a sequence of words that share statistical weight and not as a sequence of atomic queries.

%The prefix conditions the generation of the next words making the generation context aware. Variable contexts can be accounted for without strict built-in length limits. The model is robust to long-tail effects as the prefix is a sequence of words and not as a sequence of atomic queries. Finally, the generated suggestions are synthetic because our model can possibly create new queries by sampling at the word level. 
To endow our model with such capabilities, we rely on recent advances in generative natural language applications with neural networks~\cite{Bengio2013,Kyung14}. Data sparsity issues are avoided by assigning single words, queries and sequences of queries to distributed representations, i.e.~dense vectors bearing syntactic and semantic characteristics~\cite{bengio2003neural}. Our model deploys a new hierarchical neural network architecture that allows to embed a complex distribution over sequences of queries within a compact parameter space exploiting distributed representations for better generalization.

This paper makes the following contribution. We present a neural network architecture for query suggestion that is context-aware, generative, robust to long-tail, memory efficient, computationally cheap at test time and that can be trained from end-to-end on search logs. Our model is fully general and can be applied to other tasks, such as query auto-completion, or can be used to generate candidates for complex learning-to-rank models.

The rest of the paper is structured as follows. In Section 2, we present the relevant state of the art and we contrast our model with existing solutions. In Section 3, we give an intuitive overview on the structure of the model. In Section 4, we formally present the model using mathematical notation. 

%Our setting has several advantages. First, decoding is a well-studied problem and is computationally affordable. 
%Using word embeddings, we are able to share statistical weight between $n$-gram contexts and generate suggestions even for rare or unseen queries in the training data.
%Each query in the session is encoded into a real-valued vector.
%The sequence of query representations is considered, at test time, to decode a possible suggestion.
%This way, we are able condition the suggestion on an unbounded sequence of previous queries.
%Our suggestions are effectively \emph{context-aware} as they are sensitive to the order and the number of the queries that have already been submitted by the user and are not limited to the last submitted query.
%Finally, we model the notion of utility of a suggestion by training a regression model that predicts the rank of the first clicked document for each query. 
%This enables the generation of suggestions that are both contextually relevant and useful, as measured by the predicted rank of the last clicked document.

